Efficient Exact Verification of Binarized Neural Networks

Concerned with the reliability of neural networks, researchers have developed verification techniques to prove their robustness. Most verifiers work with real-valued networks. Unfortunately, the exact (complete and sound) verifiers face scalability challenges and provide no correctness guarantees due to floating point errors. We argue that Binarized Neural Networks (BNNs) provide comparable robustness and allow exact and significantly more efficient verification. We present a new system, EEV, for efficient and exact verification of BNNs. EEV consists of two parts: (i) a novel SAT solver that speeds up BNN verification by natively handling the reified cardinality constraints arising in BNN encodings; and (ii) strategies to train solver-friendly robust BNNs by inducing balanced layer-wise sparsity and low cardinality bounds, and adaptively cancelling the gradients. We demonstrate the effectiveness of EEV by presenting the first exact verification results for L-inf-bounded adversarial robustness of nontrivial convolutional BNNs on the MNIST and CIFAR10 datasets. Compared to exact verification of real-valued networks of the same architectures on the same tasks, EEV verifies BNNs hundreds to thousands of times faster, while delivering comparable verifiable accuracy in most cases.

==> big-result-table.tex <==
\begin{table*}[!hbt]
    \caption{Verification Time and Test Accuracy on MNIST and CIFAR10
    Benchmarks}
    \label{tab:all-result}
    \vskip 0.5em
    \begin{footnotesize}
        \begin{center}
            \bgroup
            \def\arraystretch{1.12}
            \input{gen/table-attack-time.tex}
            \vskip 0.5em
            \input{gen/table-attack-acc.tex}
            \egroup
        \end{center}
        \begin{tablenotes}
            \item We present results of our system on BNNs and compare against
                real-valued networks of the same architecture
                in~\cite{xiao2018training}. ``\citeauthor{xiao2018training} S''
                and ``\citeauthor{xiao2018training} L'' correspond to
                real-valued networks \texttt{conv-small} and \texttt{conv-large}
                respectively, with data taken from
                \citeauthor{xiao2018training}.  We conduct a complete evaluation
                of the large architecture while \citeauthor{xiao2018training}
                evaluate only the first 1000 images due to long build time.  We
                set $(\epsilon_0,\,\epsilon_1,\,\epsilon_2)=(0.1,\,0.2,\, 0.3)$
                for MNIST and $(\epsilon_0,\,\epsilon_1,\,\epsilon_2) =
                (2/255,\, 5 / 255,\, 8 / 255)$ for CIFAR10.
        \end{tablenotes}
    \end{footnotesize}
    \vskip -0.8em
\end{table*}

% vim: tw=80 filetype=tex foldmethod=marker foldmarker=f{{{,f}}} spell spelllang=en



==> gen/table-cmp-binmask-thin.tex <==
\begin{tabular}{llrr}
\toprule
                      &         & MNIST \hspace{1em} $\epsilon=0.1$ & CIFAR10 \hspace{1em} $\epsilon=2/255$ \\
\midrule
\multirow{2}{4.8em}{Total Sparsity} & Ternary &                              81\% &                                  82\% \\
                      & BinMask &                              84\% &                                  79\% \\
\cmidrule(lr){1-4}
\multirow{2}{4.8em}{Layer-wise Sparsity} & Ternary &               16\% 40\% 84\% 36\% &                   16\% 48\% 84\% 23\% \\
                      & BinMask &               91\% 90\% 83\% 92\% &                   84\% 85\% 79\% 87\% \\
\cmidrule(lr){1-4}
\multirow{2}{4.8em}{Mean Solve Time (sub40)} & Ternary &                           756.288 &                                 0.267 \\
                      & BinMask &                             0.002 &                                 0.003 \\
\cmidrule(lr){1-4}
\multirow{2}{4.8em}{Max Solve Time (sub40)} & Ternary &                          3600.001 &                                 5.707 \\
                      & BinMask &                             0.007 &                                 0.005 \\
\cmidrule(lr){1-4}
\multirow{2}{4.8em}{Natural Test Accuracy} & Ternary &                           97.59\% &                               54.78\% \\
                      & BinMask &                           97.35\% &                               55.22\% \\
\bottomrule
\end{tabular}


==> gen/table-cmp-mnist-mlp.tex <==
\begin{tabular}{lrr}
\toprule
{} &       MNIST-MLP & \cite{narodytska2020in} \\
\midrule
Test Accuracy     &         97.14\% &                  95.2\% \\
\#Non-zero Params &  $18\mathrm{K}$ &          $20\mathrm{K}$ \\
\bottomrule
\end{tabular}


==> gen/table-ensemble.tex <==
\begin{tabular}{lR{9ex}R{10ex}R{8ex}}
\toprule
{} & Test Accuracy & Mean Solve Time (s) & Attack Success Rate \\
\midrule
\texttt{conv-small} &       94.31\% &               0.001 &             33.58\% \\
\texttt{conv-large} &       96.36\% &               0.004 &             22.41\% \\
ensemble            &       93.32\% &               0.003 &             17.21\% \\
\bottomrule
\end{tabular}

